LESS: Label-efficient Multi-scale Learning for Cytological Whole Slide Image Screening

In computational pathology, multiple instance learning (MIL) is widely used to circumvent the computational impasse in giga-pixel whole slide image (WSI) analysis. It usually consists of two stages: patch-level feature extraction and slide-level aggregation. Recently, pretrained models or self-supervised learning have been used to extract patch features, but they suffer from low effectiveness or inefficiency due to overlooking the task-specific supervision provided by slide labels. Here we propose a weakly-supervised Label-Efficient WSI Screening method, dubbed LESS, for cytological WSI analysis with only slide-level labels, which can be effectively applied to small datasets. First, we suggest using variational positive-unlabeled (VPU) learning to uncover hidden labels of both benign and malignant patches. We provide appropriate supervision by using slide-level labels to improve the learning of patch-level features. Next, we take into account the sparse and random arrangement of cells in cytological WSIs. To address this, we propose a strategy to crop patches at multiple scales and utilize a cross-attention vision transformer (CrossViT) to combine information from different scales for WSI classification. The combination of our two steps achieves task-alignment, improving effectiveness and efficiency. We validate the proposed label-efficient method on a urine cytology WSI dataset encompassing 130 samples (13,000 patches) and FNAC 2019 dataset with 212 samples (21,200 patches). The experiment shows that the proposed LESS reaches 84.79%, 85.43%, 91.79% and 78.30% on a urine cytology WSI dataset, and 96.88%, 96.86%, 98.95%, 97.06% on FNAC 2019 dataset in terms of accuracy, AUC, sensitivity and specificity. It outperforms state-of-the-art MIL methods on pathology WSIs and realizes automatic cytological WSI cancer screening.

==> MEDIMA-template/section/fig/hyperparameter_table.tex <==
\begin{table}[]
\centering
%\vspace{-10mm}
\caption{Hyperparameter setting of models. Model structures and hyperparameters are the same as those in the original papers if not listed. Learning rates are selected based on complexity of the model and stability of the training loss curve. % \xl{This table is too small.}
}

\label{tab:hyperparameter}
\resizebox{8.8cm}{!}{%
\begin{tabular}{|c|c|ccc|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Hyperparameter\\ Setting\end{tabular}} &
  Stage $1$ &
  \multicolumn{3}{c|}{Stage $2$} \\ \cline{2-5} 
 &
  VPU/PN &
  \multicolumn{1}{c|}{MLP} &
  \multicolumn{1}{c|}{GNN/Fused GNN} &
  ViT/CrossViT \\ \hline
Batch size &
  $100$ &
  \multicolumn{3}{c|}{$128$} \\ \hline
Epochs &
  $10$ &
  \multicolumn{3}{c|}{$40$} \\ \hline
Optimizer &
  Adam &
  \multicolumn{3}{c|}{Adam} \\ \hline
\begin{tabular}[c]{@{}c@{}}Learning rate\\ (LR, initial, end)\end{tabular} &
  $1e-4$, $1.25e-5$ &
  \multicolumn{1}{c|}{$1e-2$, $5e-3$} &
  \multicolumn{1}{c|}{$4e-4$, $2e-4$} &
  $1e-6$, $5e-7$ \\ \hline
\begin{tabular}[c]{@{}c@{}}Warmup\\ ($\frac{1}{10}$ of the initial LR)\end{tabular} &
  - &
  \multicolumn{3}{c|}{$5$ (with $\frac{1}{10}$ initial learning rate)} \\ \hline
LR scheduler &
  \begin{tabular}[c]{@{}c@{}}Step\\ ($0.5$ every $2$ epochs)\end{tabular} &
  \multicolumn{1}{c|}{Cosine} &
  \multicolumn{1}{c|}{Cosine} &
  Cosine \\ \hline
Weight Decay &
  - &
  \multicolumn{2}{c|}{-} &
  $0$ \\ \hline
Drop &
  - &
  \multicolumn{2}{c|}{-} &
  $0.1$ \\ \hline
Drop path &
  - &
  \multicolumn{2}{c|}{-} &
  $0.1$ \\ \hline
\end{tabular}%
}
%\vspace{-5mm}
\end{table}

==> MEDIMA-template/section/table/main_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

\begin{table*}[h]
\centering
\caption{Results $(\%)$ of WSI screening metrics for baselines and \ours{} on the urine cytological WSI dataset. For single-scale models, $256\times 256$ patches are used as input. Mean and standard deviation are reported. Results in bold come from \ours{}.}\label{tab:main}
\subtable[{WSI-level screening with patch feature encoder that directly assigns WSI-label to patch-label and VPU.}]{\label{tab:main1}
\resizebox{\textwidth}{!}{\begin{tabular}{c|cccc|cccc}
\hline\hline
\multirow{2}{*}{Method} &
  \multicolumn{4}{c|}{PN} &
  \multicolumn{4}{c}{VPU} \\
   %[1pt]
  \cline{2-9} 
 &
  Acc &
  AUC &
  Sensitivity &
  Specificity &
  Acc &
  AUC &
  Sensitivity &
  Specificity \\
   %[1pt]
  \hline\hline 
Counting &
  $75.82_{(11.40)}$ &
  $75.39_{(7.74)}$ &
  $81.71_{(10.00)}$ &
  $76.06_{(11.09)}$ &
  $84.71_{(3.68)}$ &
  $72.91_{(4.99)}$ &
  $99.23_{(1.57)}$ &
  $59.54_{(4.60)}$ \\
  %[1pt]
MLP &
  $74.52_{(18.16)}$ &
  $74.25_{(18.45)}$ &
  $99.23_{(1.57)}$ &
  $85.54_{(20.70)}$ &
  $70.00_{(11.41)}$ &
  $70.09_{(11.97)}$ &
  $87.72_{(21.82)}$ &
  $67.56_{(15.08)}$ \\ 
   %[1pt]
  \hline
GNN &
  $76.44_{(3.34)}$ &
  $76.02_{(3.59)}$ &
  $79.71_{(6.22)}$ &
  $76.03_{(2.29)}$ &
  $82.88_{(3.64)}$ &
  $84.09_{(3.41)}$ &
  $94.04_{(3.03)}$ &
  $74.22_{(4.40)}$ \\
   %[1pt]
ViT &
  $76.03_{(2.29)}$ &
  $75.76_{(2.33)}$ &
  $79.46_{(3.87)}$ &
  $72.72_{(4.24)}$ &
  $83.36_{(2.04)}$ &
  $83.67_{(2.44)}$ &
  $88.32_{(2.54)}$ &
  $78.19_{(2.44)}$ \\
   %[1pt]
  \hline
Fused GNN &
  $80.55_{(3.03)}$ &
  $80.20_{(3.37)}$ &
  $83.01_{(5.52)}$ &
  $78.60_{(5.12)}$ &
  $83.29_{(1.50)}$ &
  $83.75_{(1.55)}$ &
  $89.28_{(2.81)}$ &
  $77.48_{(2.50)}$ \\
   %[1pt]
CrossViT &
  $78.56_{(2.49)}$ &
  $78.24_{(2.58)}$ &
  $81.29_{(3.81)}$ &
  $75.98_{(4.19)}$ &
  \bm{$ 84.79_{(2.13)}$} &
  \bm{$85.43_{(2.14)}$} &
  \bm{$91.79_{(3.19)}$} &
  \bm{$78.30_{(2.97)}$} \\
   %[1pt]
  \hline
\end{tabular}
}}
\subtable[{WSI-level screening with unsupervised learning feature encoding strategies.}]{\label{tab:main2}\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccc|cccc}
\hline\hline
\multirow{2}{*}{Method} &
  \multicolumn{4}{c|}{Pretrained model on ImageNet} &
  \multicolumn{4}{c}{SimCLR (with 50 pretrain epochs)} \\
   %[1pt]
  \cline{2-9} 
 &
  Acc &
  AUC &
  Sensitivity &
  Specificity &
  Acc &
  AUC &
  Sensitivity &
  Specificity \\
   %[1pt]
  \hline\hline 
GNN &
$74.59_{(1.04)}$&
 $74.58_{(1.08)}$&
$79.05_{(1.81)}$&
$69.72_{(1.71)}$&
 $79.67_{(1.78)}$&
 $79.86_{(1.82)}$&
$84.55_{(3.20)}$&
$74.72_{(3.02)}$ \\
   %[1pt]
ViT &
   $74.65_{(2.45)}$  &
   $74.09_{(2.88)}$  &
    $80.65_{(5.12)}$ &
    $72.00_{(2.85)}$ &
  $80.36_{(4.52)}$ &
  $78.98_{(4.61)}$ &
  $78.25_{(3.93)}$ &
  $80.47_{(8.45)}$ \\
   [1pt]
  \hline
Fused GNN &
  $75.00_{(1.66)}$ &
  $74.79_{(1.70)}$ &
  $78.52_{(1.93)}$ &
  $70.86_{(2.24)}$ &
   $80.21_{(2.20)}$ &
   $79.79_{(2.52)}$ &
  $82.02_{(3.25)}$  &
   $77.98_{(1.62)}$ \\
   %[1pt]
CrossViT &
 $75.34_{(1.78)}$ &
 $75.99_{(1.88)}$&
  $82.86_{(2.92)}$&
  $72.41_{(2.41)}$&
 $80.82_{(1.40)}$&
$80.53_{(1.45)}$&
$84.62_{(2.15)}$&
$77.78_{(2.61)}$\\
   %[1pt]
  \hline
\end{tabular}%
}}
\vspace{-5mm}
\end{table*}

%%%%%% multi-table examples
% \begin{table}
% \caption{Caption for total table}
% \centering
 
% \subtable[Table 1]{
% \begin{tabular}{ccc}
% a & b & c
% \end{tabular}
% \label{firsttable}
% }
 
% \qquad
 
% \subtable[Table 2]{        
% \begin{tabular}{ccc}
% A & B & C
% \end{tabular}
% \label{secondtable}
% }
 
% \end{table}



==> MEDIMA-template/section/table/sup_table.tex <==
\begin{table*}[h]
\centering
% \vspace{-7mm}
\caption{Results $(\%)$ of WSI-level screening with pretrained VGG16 on ImageNet and SimCLR trained with self-supervised startegy show that pretrained and unsupervised learning-based feature extractors are both worse compared to our proposed VPU as shown in Table 1 in the manuscript. $256\times 256$ patches are input for single-scale models. \xl{What's the reason for omitting counting and MLP here? What are your reasons of separating table 1 and 2?}}
% \xl{You have to give a takeaway from this table} Using unsupervised feature extractor resulted in xxxxx worse results compared with our proposed strategy as shown in Table~\ref{}.
\label{tab:sup_main}
\resizebox{\textwidth}{!}{%\textwidth
\begin{tabular}{c|cccc|cccc}
\hline\hline
\multirow{2}{*}{Method} &
  \multicolumn{4}{c|}{PN (pretrained on ImageNet)} &
  \multicolumn{4}{c}{SimCLR (with 50 pretrain epochs)} \\
   [1pt]
  \cline{2-9} 
 &
  Acc &
  AUC &
  Sensitivity &
  Specificity &
  Acc &
  AUC &
  Sensitivity &
  Specificity \\
   [1pt]
  \hline\hline 
GNN &
$74.59_{(1.04)}$&
 $74.58_{(1.08)}$&
$79.05_{(1.81)}$&
$69.72_{(1.71)}$&
 $79.67_{(1.78)}$&
 $79.86_{(1.82)}$&
$84.55_{(3.20)}$&
$74.72_{(3.02)}$ \\
   [1pt]
ViT &
   $74.65_{(2.45)}$  &
   $74.09_{(2.88)}$  &
    $80.65_{(5.12)}$ &
    $72.00_{(2.85)}$ &
  $80.36_{(4.52)}$ &
  $78.98_{(4.61)}$ &
  $78.25_{(3.93)}$ &
  $80.47_{(8.45)}$ \\
   [1pt]
  \hline
Fused GNN &
  $75.00_{(1.66)}$ &
  $74.79_{(1.70)}$ &
  $78.52_{(1.93)}$ &
  $70.86_{(2.24)}$ &
   $80.21_{(2.20)}$ &
   $79.79_{(2.52)}$ &
  $82.02_{(3.25)}$  &
   $77.98_{(1.62)}$ \\
   [1pt]
CrossViT &
 $75.34_{(1.78)}$ &
 $75.99_{(1.88)}$&
  $82.86_{(2.92)}$&
  $72.41_{(2.41)}$&
 $80.82_{(1.40)}$&
$80.53_{(1.45)}$&
$84.62_{(2.15)}$&
$77.78_{(2.61)}$\\
   [1pt]
  \hline
\end{tabular}%
}
\end{table*}

